Robust and Energy-efficient PPG-based Heart-Rate Monitoring

A wrist-worn PPG sensor coupled with a lightweight algorithm can run on a MCU to enable non-invasive and comfortable monitoring, but ensuring robust PPG-based heart-rate monitoring in the presence of motion artifacts is still an open challenge. Recent state-of-the-art algorithms combine PPG and inertial signals to mitigate the effect of motion artifacts. However, these approaches suffer from limited generality. Moreover, their deployment on MCU-based edge nodes has not been investigated. In this work, we tackle both the aforementioned problems by proposing the use of hardware-friendly Temporal Convolutional Networks (TCN) for PPG-based heart estimation. Starting from a single "seed" TCN, we leverage an automatic Neural Architecture Search (NAS) approach to derive a rich family of models. Among them, we obtain a TCN that outperforms the previous state-of-the-art on the largest PPG dataset available (PPGDalia), achieving a Mean Absolute Error (MAE) of just 3.84 Beats Per Minute (BPM). Furthermore, we tested also a set of smaller yet still accurate (MAE of 5.64 - 6.29 BPM) networks that can be deployed on a commercial MCU (STM32L4) which require as few as 5k parameters and reach a latency of 17.1 ms consuming just 0.21 mJ per inference.

==> text/Table1.tex <==
\begin{table}
\small
\centering
\caption{Transfer learning of TEMPONet architecture from sEMG bio-signal to PPG signal.}
\label{tab:morph}
\begin{tabular}{l|lll}
                      & \textbf{MAE [BPM]} & \textbf{Parameters} & \textbf{MACs} \\ \hline\hline
\textbf{TEMPO Net} & 5.78         & 429K                & 13.5M         \\
\textbf{TimePPG Net} & 5.68         & 300K                & 12.9M         \\ \hline
\end{tabular}
\end{table}

==> text/image_tables.tex <==

\input{text/Table1.tex}
\input{text/Table2.tex}
\begin{figure}
  \centering
\includegraphics[width=1.35\columnwidth]{./figures/Network_exploration.png}
  \caption{.}
  \label{fig:architecture}
\end{figure}
\input{text/Table3.tex}
\section{Background}
%
\begin{figure*}
  \centering
\includegraphics[width=0.95\textwidth]{./figures/Single_patient_trace.png}
  \caption{.}
  \label{fig:architecture}
\end{figure*}
\begin{figure*}
  \centering
\includegraphics[width=0.95\textwidth]{./figures/Framework.png}
  \caption{.}
  \label{fig:architecture}
\end{figure*}
\begin{figure}
  \centering
\includegraphics[width=0.95\columnwidth]{./figures/ActPPG_tradeoff.png}
  \caption{.}
  \label{fig:architecture}
\end{figure}
\begin{figure}
  \centering
\includegraphics[width=0.95\columnwidth]{./figures/Low_movement_windows.png}
  \caption{.}
  \label{fig:architecture}
\end{figure}
%
